High-order well-balanced finite volume schemes for the Euler equations with gravitation

A high-order well-balanced scheme for the Euler equations with gravitation is presented. The scheme is able to preserve a spatially high-order accurate discrete representation of a large class of hydrostatic equilibria. It is based on a novel local hydrostatic reconstruction, which, in combination with any standard high-order accurate reconstruction procedure, achieves genuine high-order accuracy for smooth solutions close or away from equilibrium. The resulting scheme is very simple and can be implemented into any existing finite volume code with minimal effort. Moreover, the scheme is not tied to any particular form of the equation of state, which is crucial for example in astrophysical applications. Several numerical experiments demonstrate the robustness and high-order accuracy of the scheme nearby and out of hydrostatic equilibrium.

==> img/one-dimensional/one_dimensional_equilibrium_eq-E.tex <==
\begin{tabular}{r
                S[table-format=3.2e2]r
                S[table-format=3.2e2]r
}
\toprule
N & 
\multicolumn{2}{c}{\cwenonaive} & 
\multicolumn{2}{c}{\cwenoisentropic} \\
 & 
\multicolumn{1}{c}{$err_{eq,1}(E)$} & 
\multicolumn{1}{c}{rate} & 
\multicolumn{1}{c}{$err_{eq,1}(E)$} & 
\multicolumn{1}{c}{rate} \\
\midrule
  32 &  1.63e-03  &      --  &  7.20e-16  &      --   \\
  64 &  2.51e-04  &     2.69 &  1.01e-14  &    -3.80  \\
 128 &  2.27e-05  &     3.47 &  2.66e-15  &     1.92  \\
 256 &  2.57e-06  &     3.14 &  5.44e-15  &    -1.03  \\
 512 &  3.30e-07  &     2.96 &  3.30e-15  &     0.72  \\
1024 &  4.21e-08  &     2.97 &  5.16e-15  &    -0.64  \\
\bottomrule
\end{tabular}

==> img/one-dimensional/one_dimensional_smooth_delta-E.tex <==
\begin{tabular}{r
                S[table-format=3.2e2]r
                S[table-format=3.2e2]r
}
\toprule
N & 
\multicolumn{2}{c}{\cwenonaive} & 
\multicolumn{2}{c}{\cwenoisentropic} \\
 & 
\multicolumn{1}{c}{$err_{1}(\delta E)$} & 
\multicolumn{1}{c}{rate} & 
\multicolumn{1}{c}{$err_{1}(\delta E)$} & 
\multicolumn{1}{c}{rate} \\
\midrule
  32 &  4.72e-05  &      --  &  6.97e-09  &      --   \\
  64 &  6.43e-06  &     2.88 &  1.84e-09  &     1.92  \\
 128 &  8.81e-07  &     2.87 &  3.02e-10  &     2.61  \\
 256 &  1.17e-07  &     2.91 &  4.14e-11  &     2.87  \\
 512 &  1.50e-08  &     2.96 &  5.40e-12  &     2.94  \\
1024 &  1.87e-09  &     3.01 &  6.78e-13  &     2.99  \\
\bottomrule
\end{tabular}

==> img/one-dimensional/one_dimensional_smooth_normal-E.tex <==
\begin{tabular}{r
                S[table-format=3.2e2]r
                S[table-format=3.2e2]r
}
\toprule
N & 
\multicolumn{2}{c}{\cwenonaive} & 
\multicolumn{2}{c}{\cwenoisentropic} \\
 & 
\multicolumn{1}{c}{$err_{1}(E)$} & 
\multicolumn{1}{c}{rate} & 
\multicolumn{1}{c}{$err_{1}(E)$} & 
\multicolumn{1}{c}{rate} \\
\midrule
  32 &  4.72e-05  &      --  &  8.49e-09  &      --   \\
  64 &  6.43e-06  &     2.88 &  1.94e-09  &     2.13  \\
 128 &  8.81e-07  &     2.87 &  3.09e-10  &     2.65  \\
 256 &  1.17e-07  &     2.91 &  4.19e-11  &     2.89  \\
 512 &  1.50e-08  &     2.96 &  5.43e-12  &     2.95  \\
1024 &  1.87e-09  &     3.01 &  6.78e-13  &     3.00  \\
\bottomrule
\end{tabular}

==> img/one-dimensional/one_dimensional_smooth_normal-rho.tex <==
\begin{tabular}{r
                S[table-format=3.2e2]r
                S[table-format=3.2e2]r
}
\toprule
N & 
\multicolumn{2}{c}{\cwenonaive} & 
\multicolumn{2}{c}{\cwenoisentropic} \\
 & 
\multicolumn{1}{c}{$err_{1}(\rho)$} & 
\multicolumn{1}{c}{rate} & 
\multicolumn{1}{c}{$err_{1}(\rho)$} & 
\multicolumn{1}{c}{rate} \\
\midrule
  32 &  5.84e-06  &      --  &  3.16e-09  &      --   \\
  64 &  6.19e-07  &     3.24 &  8.24e-10  &     1.94  \\
 128 &  1.79e-07  &     1.79 &  1.34e-10  &     2.61  \\
 256 &  3.37e-08  &     2.41 &  1.84e-11  &     2.87  \\
 512 &  4.90e-09  &     2.78 &  2.40e-12  &     2.94  \\
1024 &  6.24e-10  &     2.97 &  3.02e-13  &     2.99  \\
\bottomrule
\end{tabular}

==> img/polytrope/at-rest/polytrope_at_rest_eq-E.tex <==
\begin{tabular}{r
                S[table-format=3.2e2]r
                S[table-format=3.2e2]r
}
\toprule
N & 
\multicolumn{2}{c}{\cwenonaive} & 
\multicolumn{2}{c}{\cwenoisentropic} \\
 & 
\multicolumn{1}{c}{$err_{eq,1}(E)$} & 
\multicolumn{1}{c}{rate} & 
\multicolumn{1}{c}{$err_{eq,1}(E)$} & 
\multicolumn{1}{c}{rate} \\
\midrule
  32 &  4.85e-04  &      --  &  4.60e-11  &      --   \\
  64 &  5.71e-05  &     3.09 &  7.29e-13  &     5.98  \\
 128 &  6.94e-06  &     3.04 &  1.23e-14  &     5.89  \\
 256 &  8.45e-07  &     3.04 &  3.71e-15  &     1.73  \\
 512 &  1.02e-07  &     3.05 &  5.13e-15  &    -0.47  \\
1024 &  1.18e-08  &     3.11 &  6.23e-15  &    -0.28  \\
\bottomrule
\end{tabular}

==> img/polytrope/at-rest/polytrope_at_rest_normal-E.tex <==
\begin{tabular}{r
                S[table-format=3.2e2]r
                S[table-format=3.2e2]r
}
\toprule
N & 
\multicolumn{2}{c}{\cwenonaive} & 
\multicolumn{2}{c}{\cwenoisentropic} \\
 & 
\multicolumn{1}{c}{$err_{1}(E)$} & 
\multicolumn{1}{c}{rate} & 
\multicolumn{1}{c}{$err_{1}(E)$} & 
\multicolumn{1}{c}{rate} \\
\midrule
  32 &  4.85e-04  &      --  &  9.00e-09  &      --   \\
  64 &  5.71e-05  &     3.09 &  5.61e-10  &     4.01  \\
 128 &  6.94e-06  &     3.04 &  3.50e-11  &     4.00  \\
 256 &  8.45e-07  &     3.04 &  2.18e-12  &     4.00  \\
 512 &  1.02e-07  &     3.05 &  1.32e-13  &     4.04  \\
1024 &  1.18e-08  &     3.11 &  6.24e-15  &     4.41  \\
\bottomrule
\end{tabular}

==> img/polytrope/at-rest/polytrope_at_rest_normal-rho.tex <==
\begin{tabular}{r
                S[table-format=3.2e2]r
                S[table-format=3.2e2]r
}
\toprule
N & 
\multicolumn{2}{c}{\cwenonaive} & 
\multicolumn{2}{c}{\cwenoisentropic} \\
 & 
\multicolumn{1}{c}{$err_{1}(\rho)$} & 
\multicolumn{1}{c}{rate} & 
\multicolumn{1}{c}{$err_{1}(\rho)$} & 
\multicolumn{1}{c}{rate} \\
\midrule
  32 &  1.57e-03  &      --  &  2.79e-09  &      --   \\
  64 &  1.85e-04  &     3.09 &  1.73e-10  &     4.01  \\
 128 &  2.22e-05  &     3.06 &  1.08e-11  &     4.00  \\
 256 &  2.66e-06  &     3.06 &  6.72e-13  &     4.01  \\
 512 &  3.07e-07  &     3.12 &  2.07e-13  &     1.70  \\
1024 &  3.31e-08  &     3.21 &  3.94e-13  &    -0.93  \\
\bottomrule
\end{tabular}

==> img/polytrope/smooth/polytrope_smooth_huge_delta-E.tex <==
\begin{tabular}{r
                S[table-format=3.2e2]r
                S[table-format=3.2e2]r
}
\toprule
N & 
\multicolumn{2}{c}{\cwenonaive} & 
\multicolumn{2}{c}{\cwenoisentropic} \\
 & 
\multicolumn{1}{c}{$err_{1}(\delta E)$} & 
\multicolumn{1}{c}{rate} & 
\multicolumn{1}{c}{$err_{1}(\delta E)$} & 
\multicolumn{1}{c}{rate} \\
\midrule
  32 &  4.91e-02  &      --  &  5.13e-02  &      --   \\
  64 &  2.48e-02  &     0.98 &  2.57e-02  &     1.00  \\
 128 &  1.15e-02  &     1.11 &  1.18e-02  &     1.12  \\
 256 &  5.31e-03  &     1.12 &  5.41e-03  &     1.13  \\
 512 &  2.67e-03  &     0.99 &  2.69e-03  &     1.01  \\
1024 &  1.37e-03  &     0.96 &  1.37e-03  &     0.97  \\
\bottomrule
\end{tabular}

==> img/polytrope/smooth/polytrope_smooth_huge_normal-E.tex <==
\begin{tabular}{r
                S[table-format=3.2e2]r
                S[table-format=3.2e2]r
}
\toprule
N & 
\multicolumn{2}{c}{\cwenonaive} & 
\multicolumn{2}{c}{\cwenoisentropic} \\
 & 
\multicolumn{1}{c}{$err_{1}(E)$} & 
\multicolumn{1}{c}{rate} & 
\multicolumn{1}{c}{$err_{1}(E)$} & 
\multicolumn{1}{c}{rate} \\
\midrule
  32 &  4.91e-02  &      --  &  5.13e-02  &      --   \\
  64 &  2.48e-02  &     0.98 &  2.57e-02  &     1.00  \\
 128 &  1.15e-02  &     1.11 &  1.18e-02  &     1.12  \\
 256 &  5.31e-03  &     1.12 &  5.41e-03  &     1.13  \\
 512 &  2.67e-03  &     0.99 &  2.69e-03  &     1.01  \\
1024 &  1.37e-03  &     0.96 &  1.37e-03  &     0.97  \\
\bottomrule
\end{tabular}

==> img/polytrope/smooth/polytrope_smooth_huge_normal-rho.tex <==
\begin{tabular}{r
                S[table-format=3.2e2]r
                S[table-format=3.2e2]r
}
\toprule
N & 
\multicolumn{2}{c}{\cwenonaive} & 
\multicolumn{2}{c}{\cwenoisentropic} \\
 & 
\multicolumn{1}{c}{$err_{1}(\rho)$} & 
\multicolumn{1}{c}{rate} & 
\multicolumn{1}{c}{$err_{1}(\rho)$} & 
\multicolumn{1}{c}{rate} \\
\midrule
  32 &  2.88e-02  &      --  &  2.98e-02  &      --   \\
  64 &  1.42e-02  &     1.02 &  1.46e-02  &     1.03  \\
 128 &  6.37e-03  &     1.16 &  6.46e-03  &     1.17  \\
 256 &  3.02e-03  &     1.08 &  3.05e-03  &     1.08  \\
 512 &  1.51e-03  &     1.00 &  1.52e-03  &     1.01  \\
1024 &  7.74e-04  &     0.97 &  7.74e-04  &     0.97  \\
\bottomrule
\end{tabular}

==> img/polytrope/smooth/polytrope_smooth_large_delta-E.tex <==
\begin{tabular}{r
                S[table-format=3.2e2]r
                S[table-format=3.2e2]r
}
\toprule
N & 
\multicolumn{2}{c}{\cwenonaive} & 
\multicolumn{2}{c}{\cwenoisentropic} \\
 & 
\multicolumn{1}{c}{$err_{1}(\delta E)$} & 
\multicolumn{1}{c}{rate} & 
\multicolumn{1}{c}{$err_{1}(\delta E)$} & 
\multicolumn{1}{c}{rate} \\
\midrule
  32 &  1.57e-04  &      --  &  1.00e-04  &      --   \\
  64 &  3.93e-05  &     2.00 &  3.26e-05  &     1.62  \\
 128 &  6.01e-06  &     2.71 &  5.20e-06  &     2.65  \\
 256 &  7.43e-07  &     3.02 &  6.81e-07  &     2.93  \\
 512 &  9.09e-08  &     3.03 &  8.57e-08  &     2.99  \\
1024 &  1.11e-08  &     3.03 &  1.07e-08  &     2.99  \\
\bottomrule
\end{tabular}

==> img/polytrope/smooth/polytrope_smooth_large_normal-E.tex <==
\begin{tabular}{r
                S[table-format=3.2e2]r
                S[table-format=3.2e2]r
}
\toprule
N & 
\multicolumn{2}{c}{\cwenonaive} & 
\multicolumn{2}{c}{\cwenoisentropic} \\
 & 
\multicolumn{1}{c}{$err_{1}(E)$} & 
\multicolumn{1}{c}{rate} & 
\multicolumn{1}{c}{$err_{1}(E)$} & 
\multicolumn{1}{c}{rate} \\
\midrule
  32 &  1.57e-04  &      --  &  1.00e-04  &      --   \\
  64 &  3.93e-05  &     2.00 &  3.26e-05  &     1.62  \\
 128 &  6.01e-06  &     2.71 &  5.20e-06  &     2.65  \\
 256 &  7.43e-07  &     3.02 &  6.81e-07  &     2.93  \\
 512 &  9.09e-08  &     3.03 &  8.57e-08  &     2.99  \\
1024 &  1.11e-08  &     3.03 &  1.07e-08  &     2.99  \\
\bottomrule
\end{tabular}

==> img/polytrope/smooth/polytrope_smooth_large_normal-rho.tex <==
\begin{tabular}{r
                S[table-format=3.2e2]r
                S[table-format=3.2e2]r
}
\toprule
N & 
\multicolumn{2}{c}{\cwenonaive} & 
\multicolumn{2}{c}{\cwenoisentropic} \\
 & 
\multicolumn{1}{c}{$err_{1}(\rho)$} & 
\multicolumn{1}{c}{rate} & 
\multicolumn{1}{c}{$err_{1}(\rho)$} & 
\multicolumn{1}{c}{rate} \\
\midrule
  32 &  8.43e-05  &      --  &  5.50e-05  &      --   \\
  64 &  2.15e-05  &     1.97 &  1.79e-05  &     1.62  \\
 128 &  3.27e-06  &     2.72 &  2.84e-06  &     2.65  \\
 256 &  4.04e-07  &     3.02 &  3.72e-07  &     2.93  \\
 512 &  4.95e-08  &     3.03 &  4.68e-08  &     2.99  \\
1024 &  6.14e-09  &     3.01 &  5.87e-09  &     3.00  \\
\bottomrule
\end{tabular}

==> img/polytrope/smooth/polytrope_smooth_medium_delta-E.tex <==
\begin{tabular}{r
                S[table-format=3.2e2]r
                S[table-format=3.2e2]r
}
\toprule
N & 
\multicolumn{2}{c}{\cwenonaive} & 
\multicolumn{2}{c}{\cwenoisentropic} \\
 & 
\multicolumn{1}{c}{$err_{1}(\delta E)$} & 
\multicolumn{1}{c}{rate} & 
\multicolumn{1}{c}{$err_{1}(\delta E)$} & 
\multicolumn{1}{c}{rate} \\
\midrule
  32 &  1.07e-04  &      --  &  9.14e-07  &      --   \\
  64 &  1.20e-05  &     3.16 &  2.88e-07  &     1.67  \\
 128 &  1.07e-06  &     3.48 &  5.01e-08  &     2.52  \\
 256 &  9.31e-08  &     3.53 &  6.75e-09  &     2.89  \\
 512 &  8.49e-09  &     3.45 &  8.55e-10  &     2.98  \\
1024 &  8.13e-10  &     3.39 &  1.07e-10  &     3.00  \\
\bottomrule
\end{tabular}

==> img/polytrope/smooth/polytrope_smooth_medium_normal-E.tex <==
\begin{tabular}{r
                S[table-format=3.2e2]r
                S[table-format=3.2e2]r
}
\toprule
N & 
\multicolumn{2}{c}{\cwenonaive} & 
\multicolumn{2}{c}{\cwenoisentropic} \\
 & 
\multicolumn{1}{c}{$err_{1}(E)$} & 
\multicolumn{1}{c}{rate} & 
\multicolumn{1}{c}{$err_{1}(E)$} & 
\multicolumn{1}{c}{rate} \\
\midrule
  32 &  1.07e-04  &      --  &  9.16e-07  &      --   \\
  64 &  1.20e-05  &     3.16 &  2.88e-07  &     1.67  \\
 128 &  1.07e-06  &     3.48 &  5.01e-08  &     2.52  \\
 256 &  9.31e-08  &     3.53 &  6.75e-09  &     2.89  \\
 512 &  8.49e-09  &     3.45 &  8.55e-10  &     2.98  \\
1024 &  8.13e-10  &     3.39 &  1.07e-10  &     3.00  \\
\bottomrule
\end{tabular}

==> img/polytrope/smooth/polytrope_smooth_medium_normal-rho.tex <==
\begin{tabular}{r
                S[table-format=3.2e2]r
                S[table-format=3.2e2]r
}
\toprule
N & 
\multicolumn{2}{c}{\cwenonaive} & 
\multicolumn{2}{c}{\cwenoisentropic} \\
 & 
\multicolumn{1}{c}{$err_{1}(\rho)$} & 
\multicolumn{1}{c}{rate} & 
\multicolumn{1}{c}{$err_{1}(\rho)$} & 
\multicolumn{1}{c}{rate} \\
\midrule
  32 &  5.76e-05  &      --  &  5.01e-07  &      --   \\
  64 &  6.27e-06  &     3.20 &  1.58e-07  &     1.67  \\
 128 &  5.46e-07  &     3.52 &  2.74e-08  &     2.52  \\
 256 &  4.70e-08  &     3.54 &  3.69e-09  &     2.89  \\
 512 &  4.84e-09  &     3.28 &  4.67e-10  &     2.98  \\
1024 &  5.67e-10  &     3.09 &  5.86e-11  &     3.00  \\
\bottomrule
\end{tabular}

==> img/polytrope/smooth/polytrope_smooth_small_delta-E.tex <==
\begin{tabular}{r
                S[table-format=3.2e2]r
                S[table-format=3.2e2]r
}
\toprule
N & 
\multicolumn{2}{c}{\cwenonaive} & 
\multicolumn{2}{c}{\cwenoisentropic} \\
 & 
\multicolumn{1}{c}{$err_{1}(\delta E)$} & 
\multicolumn{1}{c}{rate} & 
\multicolumn{1}{c}{$err_{1}(\delta E)$} & 
\multicolumn{1}{c}{rate} \\
\midrule
  32 &  1.06e-04  &      --  &  9.15e-11  &      --   \\
  64 &  1.18e-05  &     3.17 &  2.88e-11  &     1.67  \\
 128 &  1.05e-06  &     3.49 &  5.03e-12  &     2.52  \\
 256 &  9.16e-08  &     3.52 &  6.94e-13  &     2.86  \\
 512 &  8.52e-09  &     3.43 &  1.07e-13  &     2.69  \\
1024 &  8.13e-10  &     3.39 &  4.10e-14  &     1.39  \\
\bottomrule
\end{tabular}

==> img/polytrope/smooth/polytrope_smooth_small_normal-E.tex <==
\begin{tabular}{r
                S[table-format=3.2e2]r
                S[table-format=3.2e2]r
}
\toprule
N & 
\multicolumn{2}{c}{\cwenonaive} & 
\multicolumn{2}{c}{\cwenoisentropic} \\
 & 
\multicolumn{1}{c}{$err_{1}(E)$} & 
\multicolumn{1}{c}{rate} & 
\multicolumn{1}{c}{$err_{1}(E)$} & 
\multicolumn{1}{c}{rate} \\
\midrule
  32 &  1.06e-04  &      --  &  8.96e-09  &      --   \\
  64 &  1.18e-05  &     3.17 &  5.60e-10  &     4.00  \\
 128 &  1.05e-06  &     3.49 &  3.50e-11  &     4.00  \\
 256 &  9.16e-08  &     3.52 &  2.20e-12  &     3.99  \\
 512 &  8.52e-09  &     3.43 &  1.57e-13  &     3.81  \\
1024 &  8.13e-10  &     3.39 &  6.08e-14  &     1.37  \\
\bottomrule
\end{tabular}

==> img/polytrope/smooth/polytrope_smooth_small_normal-rho.tex <==
\begin{tabular}{r
                S[table-format=3.2e2]r
                S[table-format=3.2e2]r
}
\toprule
N & 
\multicolumn{2}{c}{\cwenonaive} & 
\multicolumn{2}{c}{\cwenoisentropic} \\
 & 
\multicolumn{1}{c}{$err_{1}(\rho)$} & 
\multicolumn{1}{c}{rate} & 
\multicolumn{1}{c}{$err_{1}(\rho)$} & 
\multicolumn{1}{c}{rate} \\
\midrule
  32 &  5.74e-05  &      --  &  2.76e-09  &      --   \\
  64 &  6.20e-06  &     3.21 &  1.73e-10  &     4.00  \\
 128 &  5.34e-07  &     3.54 &  1.10e-11  &     3.98  \\
 256 &  4.69e-08  &     3.51 &  8.11e-13  &     3.76  \\
 512 &  4.84e-09  &     3.28 &  7.82e-14  &     3.37  \\
1024 &  5.67e-10  &     3.09 &  4.19e-14  &     0.90  \\
\bottomrule
\end{tabular}

==> img/white_dwarf/white_dwarf_eq-E.tex <==
\begin{tabular}{r
                S[table-format=3.2e2]r
                S[table-format=3.2e2]r
}
\toprule
N & 
\multicolumn{2}{c}{\cwenonaive} & 
\multicolumn{2}{c}{\cwenoisentropic} \\
 & 
\multicolumn{1}{c}{$err_{eq,1}(E)$} & 
\multicolumn{1}{c}{rate} & 
\multicolumn{1}{c}{$err_{eq,1}(E)$} & 
\multicolumn{1}{c}{rate} \\
\midrule
 128 &  3.49e+23  &      --  &  9.30e+12  &      --   \\
\bottomrule
\end{tabular}

==> img/white_dwarf/white_dwarf_eq-rho.tex <==
\begin{tabular}{r
                S[table-format=3.2e2]r
                S[table-format=3.2e2]r
}
\toprule
N & 
\multicolumn{2}{c}{\cwenonaive} & 
\multicolumn{2}{c}{\cwenoisentropic} \\
 & 
\multicolumn{1}{c}{$err_{eq,1}(\rho)$} & 
\multicolumn{1}{c}{rate} & 
\multicolumn{1}{c}{$err_{eq,1}(\rho)$} & 
\multicolumn{1}{c}{rate} \\
\midrule
 128 &  2.87e+05  &      --  &  8.67e-06  &      --   \\
\bottomrule
\end{tabular}
